FocusNet: Transformer-enhanced Polyp Segmentation with Local and Pooling Attention

Colonoscopy is vital in the early diagnosis of colorectal polyps. Regular screenings can effectively prevent benign polyps from progressing to CRC. While deep learning has made impressive strides in polyp segmentation, most existing models are trained on single-modality and single-center data, making them less effective in real-world clinical environments. To overcome these limitations, we propose FocusNet, a Transformer-enhanced focus attention network designed to improve polyp segmentation. FocusNet incorporates three essential modules: the Cross-semantic Interaction Decoder Module (CIDM) for generating coarse segmentation maps, the Detail Enhancement Module (DEM) for refining shallow features, and the Focus Attention Module (FAM), to balance local detail and global context through local and pooling attention mechanisms. We evaluate our model on PolypDB, a newly introduced dataset with multi-modality and multi-center data for building more reliable segmentation methods. Extensive experiments showed that FocusNet consistently outperforms existing state-of-the-art approaches with a high dice coefficients of 82.47% on the BLI modality, 88.46% on FICE, 92.04% on LCI, 82.09% on the NBI and 93.42% on WLI modality, demonstrating its accuracy and robustness across five different modalities. The source code for FocusNet is available at https://github.com/JunZengz/FocusNet.

==> takeout.tex <==

%Its incidence rises rapidly with age, doubling approximately every five years before age 50 and increasing by approximately 30\% in subsequent cohorts aged 55 and older~\cite{siegel2024cancer}. More than 90\% of CRC cases are diagnosed
%in individuals over the age of 50, with the average age at
%diagnosis being 64~\cite{amersi2005colorectal}. Risk factors like smoking, alcohol intake, poor diet, and physical inactivity are strongly associated with the development of this disease~\cite{islami2018proportion}.

%Approximately 90\% of CRC cases are diagnosed in individuals over the age of 50, with the average age at diagnosis being 64. 



 %Some samples from different modalities are presented in  Figure~\ref{fig:SampleswithDiffModalities}.

%In this paper, we propose \ourmodel, a novel focus attention network for robust polyp segmentation, which utilizes PVTv2 to generate hierarchical features. Then CIDM module is utilized to generate the contextual feature and coarse segmentation map. Simultaneously, FocusNet utilizes the DEM module to enhance the low-level features. Finally, the FAM module is performed to refine boundary information by simulating the process of human vision processing. Our contributions can be summarized as follows:

%Wang et al.~\cite{wang2020eca} introduced an efficient channel attention mechanism that employs a local cross-channel interaction strategy, which brings clear improvements without increasing model complexity. These attention modules are lightweight, plug-and-play blocks that can be easily integrated into the network to improve performance. 

%Hu et al.~\cite{hu2018squeeze} proposed the Squeeze-and-Excitation block, which recalibrates channel responses and enhances the network's representational capability by modeling inter-channel dependencies. Woo et al.~\cite{woo2018cbam} introduced the convolutional block attention module to enhance feature selection and optimize feature representation by leveraging both channel and spatial attention mechanisms. 

	%\scriptsize
	%\renewcommand{\arraystretch}{1.4}
   % \resizebox{\columnwidth}{!}{
	%\setlength\tabcolsep{13pt}
